Auto-Positioning in Radio-based Localization Systems: A Bayesian Approach

The application of radio-based positioning systems is ever increasing. In light of the dissemination of the Internet of Things and location-aware communication systems, the demands on localization architectures and amount of possible use cases steadily increases. While traditional radio-based localization is performed by utilizing stationary nodes, whose positions are absolutely referenced, collaborative auto-positioning methods aim to estimate location information without any a-priori knowledge of the node distribution. The usage of auto-positioning decreases the installation efforts of localization systems and therefore allows their market-wide dissemination. Since observations and position information in this scenario are correlated, the uncertainties of all nodes need to be considered. In this paper we propose a discrete Bayesian method based on a multi-dimensional histogram filter to solve the task of robust auto-positioning, allowing to propagate historical positions and estimated position uncertainties, as well as lowering the demands on observation availability when compared to conventional closed-form approaches. The proposed method is validated utilizing different multipath-, outlier and failure-corrupted ranging measurements in a static environment, where we obtain at least 58% higher positioning accuracy compared to a baseline closed-form auto-positioning approach.

==> fig/markov_algorithm.tex <==
\begin{algorithm}[ht]
%\begin{center} \textbf{Prediction} \end{center}
\vspace{0.1cm}
%\vspace{0.1cm}
    \For{\upshape{receivers} $m$ }
    {
     \For{\upshape{grid cells} $i$}
        {\vspace{0.1cm}
            {
                $\boldsymbol{d}_{m, i}^{\text{r}} = \left \|\boldsymbol{X}^{\text{Tx}} - \boldsymbol{X}_i\right \|_2 + \left \|\boldsymbol{X}^{\text{Rx}}_m - \boldsymbol{X}_i\right \|_2 $ \\
            
        \For{\upshape{CIR samples} $n$ } 
    {
            \vspace{0.1cm}
            $d_{m, n}^{\text{r}} = \tau_{m, n} \cdot c$ \Comment*[r]{Distance-equivalent of CIR time sample.}
            \vspace{0.1cm}
            $\boldsymbol{y}_{m, i, n}^{\text{r}} = \boldsymbol{d}_{m, n}^{\text{r}} - \boldsymbol{d}_{m, i}^{\text{r}} $\\
        }
        \vspace{0.1cm}
        $\boldsymbol{P}(\mathcal{\boldsymbol{Z}}|\boldsymbol{X}_i) \leftarrow \alpha_{m, n} \cdot \mathcal{N}(\boldsymbol{y}_{m, i}^{\text{r}}, \Sigma^{\text{r}})$ \Comment*[r]{Magnitude-weighted sampling.}
        }
    }
    }
    \caption{Probability Grid Mapping - Likelihood Calculation.}
    \label{alg:grid_mapping}
\end{algorithm}
